Time-Reversible Bridges of Data with Machine Learning

The analysis of dynamical systems is a fundamental tool in the natural sciences and engineering. It is used to understand the evolution of systems as large as entire galaxies and as small as individual molecules. With predefined conditions on the evolution of dy-namical systems, the underlying differential equations have to fulfill specific constraints in time and space. This class of problems is known as boundary value problems. This thesis presents novel approaches to learn time-reversible deterministic and stochastic dynamics constrained by initial and final conditions. The dynamics are inferred by machine learning algorithms from observed data, which is in contrast to the traditional approach of solving differential equations by numerical integration. The work in this thesis examines a set of problems of increasing difficulty each of which is concerned with learning a different aspect of the dynamics. Initially, we consider learning deterministic dynamics from ground truth solutions which are constrained by deterministic boundary conditions. Secondly, we study a boundary value problem in discrete state spaces, where the forward dynamics follow a stochastic jump process and the boundary conditions are discrete probability distributions. In particular, the stochastic dynamics of a specific jump process, the Ehrenfest process, is considered and the reverse time dynamics are inferred with machine learning. Finally, we investigate the problem of inferring the dynamics of a continuous-time stochastic process between two probability distributions without any reference information. Here, we propose a novel criterion to learn time-reversible dynamics of two stochastic processes to solve the Schr\"odinger Bridge Problem.

==> chapters/chapterMDHamiltonians.tex <==
\chapter{Reconstruction of Nonadiabatic Molecular Dynamics Hamiltonians}
This section determines the requirements necessary for X. This includes the functional aspects, namely Y and Z, and the non functional aspects such as A and B.

\section{Molecular Dynamics Hamiltonians}

In this chapter you will describe the requirements for your component. Try to group the requirements into subsections such as 'technical requirements', 'functional requirements', 'social requirements' or something like this. If your component consist of different partial components you can also group the requirements for the corresponding parts.

Explain the source of the requirements.

Example: The requirements for an X have been widely investigated by Organization Y.

In his paper about Z, Mister X outlines the following requirements for a Component X.

\section{Interpolation Algorithms}

\section{Experiments}

\section{Limitations \& Discussion}

==> misc/acronyms.tex <==
\addchap{List of Acronyms}

\begin{tabbing}
spacespacespace \= space \kill
3GPP	 \> 	3rd Generation Partnership Project	 \\
AJAX	\>	Asynchronous JavaScript and XML \\
API	 \> 	Application Programming Interface	 \\
AS	\>	Application Server \\
CSCF	 \> 	Call Session Control Function	 \\
CSS	\>	Cascading Stylesheets \\
DHTML	\>	Dynamic HTML \\
DOM	\>	Document Object Model \\
FOKUS	\>	Fraunhofer Institut fuer offene Kommunikationssysteme \\
GUI	\>	Graphical User Interface \\
GPS	\>	Global Positioning System \\
GSM	\>	Global System for Mobile Communication\\
HTML	\>	Hypertext Markup Language \\
HSS	 \> 	Home Subscriber Server	 \\
HTTP	 \> 	Hypertext Transfer Protocol	 \\
I-CSCF	 \> 	Interrogating-Call Session Control Function	 \\
IETF	\>	Internet Engineering Task Force \\
IM	\>	Instant Messaging \\
IMS	 \> 	IP Multimedia Subsystem	 \\
IP	 \> 	Internet Protocol	 \\
J2ME	\>	Java Micro Edition \\
JDK	\>	Java Developer Kit \\
JRE	\>	Java Runtime Environment \\
JSON	\>	JavaScript Object Notation \\
JSR	\>	Java Specification Request \\
JVM	 \> 	Java Virtual Machine	 \\
NGN	 \> 	Next Generation Network	 \\
OMA	 \> 	Open Mobile Alliance	 \\
P-CSCF	 \> 	Proxy-Call Session Control Function	 \\
PDA	\>	Personal Digital Assistant \\
PEEM	 \> 	Policy Evaluation, Enforcement and Management	 \\
QoS	 \> 	Quality of Service	 \\
S-CSCF	 \> 	Serving-Call Session Control Function	 \\
SDK	\>	Software Developer Kit \\
SDP	\>	Session Description Protocol \\
SIP	 \> 	Session Initiation Protocol	 \\
SMS	\>	Short Message Service \\
SMSC	\> Short Message Service Center \\
SOAP	 \> 	Simple Object Access Protocol	 \\
SWF	\>	Shockwave Flash \\
SWT	\>	Standard Widget Toolkit \\
TCP	 \> 	Transmission Control Protocol	 \\
Telco API	\>	Telecommunication API \\
TLS	\>	Transport Layer Security \\
UMTS	 \> 	Universal Mobile Telecommunication System	 \\
URI	 \> 	Uniform Resource Identifier	 \\
VoIP	 \> 	Voice over Internet Protocol	 \\
W3C	 \> 	World Wide Web Consortium	 \\
WSDL	\>	Web Service Description Language \\
XCAP	 \> 	XML Configuration Access Protocol	 \\
XDMS	 \> 	XML Document Management Server	 \\
XML	 \> 	Extensible Markup Language	 \\
\end{tabbing}
\endinput


==> misc/annex.tex <==
\addchap{Annex}

\begin{appendix}

\lstset{language=,caption=Sourcecode Listing,captionpos=b,
label=yahoowidgetkon,showstringspaces=false,
basicstyle={\fontfamily{pcr}\selectfont\footnotesize}}
\begin{lstlisting}
<?xml version="1.0" encoding="UTF-8"?>
<widget>
	 <debug>off</debug>
	 <window name="myWindow" title="Hello Widget" visible="true">
		 <height>120</height>
		 <width>320</width>
		 <image src="Resources/orangebg.png">
			<name>orangebg</name>
			<hOffset>0</hOffset>
			<vOffset>0</vOffset>
		</image>
		 <text>
			 <name>myText</name>
			 <data>Hello Widget</data>
			 <color>#000000</color>
			 <size>20</size>
			 <vOffset>50</vOffset>
			 <hOffset>120</hOffset>
		 </text>
	</window>
</widget>
\end{lstlisting}

\newpage


\lstset{caption=SIP request and response packet\cite{SIPBook},
captionpos=b,label=sippacket,showstringspaces=false,
basicstyle={\fontfamily{pcr}\selectfont\footnotesize}}
\begin{lstlisting}
INVITE sip:bob@network.org SIP/2.0
Via: SIP/2.0/UDP 100.101.102.103:5060;branch=z9hG4bKmp17a
Max-Forwards: 70
To: Bob <sip:bob@network.org>
From: Alice <sip:alice@ims-network.org>;tag=42
Call-ID: 10@100.101.102.103
CSeq: 1 INVITE
Subject: How are you?
Contact: <sip:xyz@network.org>
Content-Type: application/sdp
Content-Length: 159
v=0
o=alice 2890844526 2890844526 IN IP4 100.101.102.103
s=Phone Call
t=0 0
c=IN IP4 100.101.102.103
m=audio 49170 RTP/AVP 0
a=rtpmap:0 PCMU/8000

SIP/2.0 200 OK
Via: SIP/2.0/UDP proxy.network.org:5060;branch=z9hG4bK83842.1
;received=100.101.102.105
Via: SIP/2.0/UDP 100.101.102.103:5060;branch=z9hG4bKmp17a
To: Bob <sip:bob@network.org>;tag=314159
From: Alice <sip:alice@network.org>;tag=42
Call-ID: 10@100.101.102.103
CSeq: 1 INVITE
Contact: <sip:foo@network.org>
Content-Type: application/sdp
Content-Length: 159
v=0
o=bob 2890844526 2890844526 IN IP4 200.201.202.203
s=Phone Call
c=IN IP4 200.201.202.203
t=0 0
m=audio 49172 RTP/AVP 0
a=rtpmap:0 PCMU/8000
\end{lstlisting}


\end{appendix}

\endinput


==> misc/glossary.tex <==

\begin{longtable}{p{0.2\textwidth} p{0.9\textwidth}}
	% \hline
	\textbf{Term} & \textbf{Definition}                      \\
	\hline
	$p_t(x)$      & The probability of state $x$ at time $t$ \\
	ODE           & Ordinary differential equation           \\
	SDE           & Stochastic differential equation         \\
	PDE           & Stochastic differential equation         \\
	CNN           & Convoluted neural network                \\
	RNN           & Recurrent neural network                 \\
	\hline
\end{longtable}
